VST-Flow: Fine-grained low-level reasoning about real-world C code

We show how support for information-flow security proofs could be added on top of the Verified Software Toolchain (VST). We discuss several attempts to define information flow security in a VST-compatible way, and present a statement of information flow security in "continuation-passing" style. Moreover, we present Hoare rules augmented with information flow control assertions, and sketch how these rules could be proven sound with respect to the definition given before. We also discuss how this can be implemented in the Coq proof assistant, and how VST's proof automation framework (VST-Floyd) can be adapted to support convenient information flow security proofs.

==> ifc-seq-skip.tex <==
%Axiom ifc_seq_skip:
%  forall Delta P N A c P' N' A',
%  ifc_def T Delta P N A c P' N' A' <-> ifc_def T Delta P N A (Ssequence c Sskip) P' N' A'.
%


==> ifc-skip.tex <==
%Axiom ifc_skip:
%  forall Delta P N A,
%  ifc_def T Delta P N A Sskip (lft1 normal_ret_assert P) (normalPostClsf N) (normalPostClsf A).
%


==> ifc-store-canon.tex <==

\[
\inference[\textsc{ifc-store}]{}{}
\]

%Axiom ifc_store:
%    forall Delta sh n (p: T -> val) P Q R (e1 e2 : expr)
%      (t: type) (v0: T -> val) (v v_new: T -> reptype t)
%      (l1 l2: T -> label) (N: T -> stack_clsf) (A: T -> heap_clsf),
%      (* VST preconditions: *)
%      typeof e1 = t ->
%      type_is_by_value t = true ->
%      type_is_volatile t = false ->
%      (forall x, nth_error (R x) n = Some (data_at sh t (v x) (p x))) ->
%      (forall x, ENTAIL Delta, PROPx (P x) (LOCALx (Q x) (SEPx (R x))) |--
%                 local (`(eq (p x)) (eval_lvalue e1))) ->
%      (forall x, ENTAIL Delta, PROPx (P x) (LOCALx (Q x) (SEPx (R x))) |--
%                 local (`(eq (v0 x)) (eval_expr (Ecast e2 t)))) ->
%      (forall x, JMeq (v0 x) (v_new x)) ->
%      writable_share sh ->
%      (forall x, ENTAIL Delta, PROPx (P x) (LOCALx (Q x) (SEPx (R x))) |--
%         (tc_lvalue Delta e1) && 
%         (tc_expr Delta (Ecast e2 t))) ->
%      (* IFC preconditions: *)
%      (forall x, ENTAIL Delta, PROPx (P x) (LOCALx (Q x) (SEPx (R x))) |--
%                 !! (clsf_lvalue (N x) e1 = Some (l1 x) /\
%                     clsf_expr   (N x) e2 = Some (l2 x))) ->
%      ifc_def T Delta
%        (fun x => (|>PROPx (P x) (LOCALx (Q x) (SEPx (R x)))))
%        N
%        A
%        (Sassign e1 e2)
%        (fun x => (normal_ret_assert (PROPx (P x)
%                                     (LOCALx (Q x)
%                                     (SEPx (replace_nth n (R x) (data_at sh t (v_new x) (p x))))))))
%        (normalPostClsf N)
%        (normalPostClsf (fun x loc =>
%           if heap_loc_eq_val loc (p x) then lub (l1 x) (l2 x) else A x loc)).
%

